A High-Resolution View of Fast Radio Burst Host Environments

We present Hubble Space Telescope (HST/WFC3) ultraviolet and infrared observations of eight fast radio burst (FRB) host galaxies with sub-arcsecond localizations, including the hosts of three known repeating FRBs. We quantify their spatial distributions and locations with respect to their host galaxy light distributions, finding that they occur at moderate host normalized-offsets of 1.4 $r_e$ ([0.6,2.1] $r_e$; 68% interval), occur on fainter regions of their hosts in terms of IR light, but overall trace the radial distribution of IR light in their galaxies. The FRBs in our tested distribution do not clearly trace the distributions of any other transient population with known progenitors, and are statistically distinct from the locations of LGRBs, H-poor SLSNe, SGRBs, and Ca-rich transients. We further find that most FRBs are not in regions of elevated local star formation rate and stellar mass surface densities in comparison to the mean global values of their hosts. We also place upper limits to the IR flux at the FRB positions of $m_{\rm IR}\gtrsim\!24.8-27.6$~AB~mag, constraining both satellite and background galaxies to luminosities well below the host luminosity of FRB121102. We find that 5/8 FRB hosts exhibit clear spiral arm features in IR light, and that the positions of all well-localized FRBs located in such hosts are consistent with their spiral arms, although not on their brightest regions. Our results do not strongly support the primary progenitor channel of FRBs being connected either with the most massive (stripped-envelope) stars, or with events which require kicks and long delay times (neutron star mergers).

==> figures/tab_derivedIR.tex <==
\begin{deluxetable*}{cccccccccccccccc}
\tablewidth{0pc}
\tablecaption{Derived Properties from IR Observations of Host Galaxies\label{tab:IRproperties}}
\tabletypesize{\normalsize}
\tablehead{\colhead{FRB}  
& \colhead{Filter} 
& \colhead{$r_e$ (Isophotal)}  
& \colhead{$r_e$ ({\tt GALFIT})}  
& \colhead{Host Magnitude}  
& \colhead{Limit}  
& \colhead{$A_\lambda$}  
& \colhead{$\mu_{\rm FRB}$}  
& \colhead{$\Sigma_{M*(FRB)}$}  
\\ 
&  &  (kpc) & (kpc) & (AB mag) & (AB mag) & (mag) & ($\mu$Jy arcsec$^{-2}$) 
& ($10^8 \, M_\odot \rm \, kpc^{-2})$ 
} 
\startdata 
121102& F160W& 0.99 $\pm$ 0.07& 2.05 $\pm$ 0.11& 23.435 $\pm$ 0.055& 27.4& 0.40& 14.57 $\pm$ 0.20& 0.130 $\pm$ 0.002\\ 
180916& F110W& 2.52 $\pm$ 0.15& 6.00 $\pm$ 0.01& 16.178 $\pm$ 0.005& 25.4& 0.88& 31.00 $\pm$ 0.10& 0.115 $\pm$ 0.000\\ 
180924& F160W& 2.54 $\pm$ 0.41& 2.82 $\pm$ 0.53& 19.349 $\pm$ 0.002& 26.2& 0.01& 20.69 $\pm$ 0.10& 0.810 $\pm$ 0.010\\ 
190102& F160W& 4.87 $\pm$ 0.34& 5.00 $\pm$ 0.15& 20.550 $\pm$ 0.006& 27.1& 0.11& 11.10 $\pm$ 0.11& 0.093 $\pm$ 0.002\\ 
190608& F160W& 2.65 $\pm$ 0.53& 7.37 $\pm$ 0.06& 16.693 $\pm$ 0.001& 25.2& 0.02& 17.80 $\pm$ 0.10& 0.340 $\pm$ 0.001\\ 
190711& F160W& 2.88 $\pm$ 0.32& 2.48 $\pm$ 0.13& 22.899 $\pm$ 0.014& 27.6& 0.07& 6.17 $\pm$ 0.11& 0.045 $\pm$ 0.004\\ 
190714& F160W& 4.07 $\pm$ 0.35& 3.85 $\pm$ 0.03& 18.896 $\pm$ 0.002& 25.9& 0.03& 18.00 $\pm$ 0.10& 1.752 $\pm$ 0.018\\ 
191001& F160W& 6.05 $\pm$ 0.66& 6.23 $\pm$ 0.04& 17.135 $\pm$ 0.001& 24.8& 0.01& 7.99 $\pm$ 0.10& 0.322 $\pm$ 0.007\\ 
\hline 
\enddata 
\tablecomments{Magnitudes are not corrected for Galactic extinction in the direction of the FRB 
($A_\lambda$). Limits correspond to $5\sigma$ confidence.} 
 \end{deluxetable*} 


==> figures/tab_derivedUV.tex <==
\begin{deluxetable*}{cccccccccccccccc}
\tablewidth{0pc}
\tablecaption{Derived Properties from UV Observations of Host Galaxies\label{tab:UVproperties}}
\tabletypesize{\normalsize}
\tablehead{\colhead{FRB}  
& \colhead{Filter} 
& \colhead{Host Magnitude}  
& \colhead{$A_\lambda$}  
& \colhead{$\mu_{\rm FRB}$}  
& \colhead{$\Sigma_{\rm SFR(FRB)}$}  
\\&  &  (AB mag) & (mag) & ($\mu$Jy arcsec$^{-2}$) 
& ($M_\odot \rm \, yr^{-1} \, kpc^{-2})$ 
} 
\startdata 
121102& F763M& TO BE ENTERED& 4.77& 38.00 $\pm$ 2.540 & 4.089 $\pm$ 0.818\\ 
180924& F300X& 23.478 $\pm$ 0.058& 0.12& $<$ 0.85 & $<$ 0.006\\ 
190102& F300X& $>$ 27.200& 1.40& $<$ 2.58 & $<$ 0.016\\ 
190608& F300X& 19.765 $\pm$ 0.014& 0.30& 1.73 $\pm$ 0.033 & 0.007 $\pm$ 0.001\\ 
190711& F300X& 25.008 $\pm$ 0.121& 0.88& $<$ 1.61 & $<$ 0.016\\ 
190714& F300X& 23.072 $\pm$ 0.053& 0.39& $<$ 1.12 & $<$ 0.006\\ 
191001& F300X& 21.228 $\pm$ 0.020& 0.18& $<$ 0.88 & $<$ 0.005\\ 
\hline 
\enddata 
\tablecomments{Magnitudes are not corrected for Galactic extinction in the direction of the FRB 
($A_\lambda$). Limits correspond to $5\sigma$ confidence.} 
 \end{deluxetable*} 


==> figures/tab_frbs.tex <==
\begin{deluxetable*}{cccccccc}
\tablewidth{0pc}
\tablecaption{FRB Sample and Localizations\label{tab:frbs}}
\tabletypesize{\normalsize}
\tablehead{\colhead{FRB}  
& \colhead{RA$_{\rm FRB}$} & \colhead{Dec$_{\rm FRB}$}  
& \colhead{$a_{\rm stat}$} & \colhead{$a_{\rm sys}$} 
& \colhead{$b_{\rm stat}$} & \colhead{$b_{\rm sys}$} 
& \colhead{PA} 
\\& (J2000) & (J2000) &  ($''$) & ($''$) & ($''$) & ($''$) & (deg)  
} 
\startdata 
121102& 82.994589& $33.1479316$& 0.004& 0.00& 0.002& 0.00& 90.0\\ 
180916& 29.503126& $65.7167542$& 0.001& 0.00& 0.001& 0.00& 0.0\\ 
180924& 326.105229& $-40.9000278$& 0.07& 0.09& 0.06& 0.07& 0.0\\ 
190102& 322.415667& $-79.4756944$& 0.21& 0.52& 0.17& 0.44& 0.0\\ 
190608& 334.019875& $-7.8982500$& 0.19& 0.19& 0.18& 0.18& 90.0\\ 
190611& 320.745458& $-79.3975833$& 0.34& 0.60& 0.32& 0.60& 0.0\\ 
190711& 329.419500& $-80.3580000$& 0.12& 0.38& 0.07& 0.32& 90.0\\ 
190714& 183.979667& $-13.0210278$& 0.17& 0.32& 0.10& 0.23& 90.0\\ 
191001& 323.351554& $-54.7477389$& 0.13& 0.11& 0.08& 0.10& 90.0\\ 
200430& 229.706417& $12.3768889$& 0.01& 0.02& 0.24& 1.00& 0.0\\ 
\hline 
\enddata 
\tablecomments{$a_{\rm stat}, a_{\rm sys}$ are the angular size of the semi-major axis describing the $1\sigma$ statistical and systematic uncertainties respectively.
$b$ refers to the semi-minor axis.  PA is the sky position angle of the error ellipse.
Sources without reported systematic error have been incorporated in the statistical.
Data from \cite{Day20,Tendulkar17,Marcote20,Heintz20}.}
\end{deluxetable*} 


==> figures/tab_offsets.tex <==
\begin{deluxetable*}{cccccccccccccccc}
\tablewidth{0pc}
\tablecaption{Offsets and Light Locations of FRBs\label{tab:locations}}
\tabletypesize{\normalsize}
\tablehead{\colhead{FRB}  
& \colhead{Filter} & \colhead{\angoff} & \colhead{\physoff} 
& \colhead{\physoff/\reff} & \colhead{\FF} & \colhead{\FE} 
\\&  &  ($''$) & (kpc) &  &  
} 
\startdata 
121102& F160W& 0.23 $\pm$ 0.02& 0.75$ \pm$ 0.05& 0.37 $ \pm$ 0.02& 0.70 $\pm$ 0.07&0.24 $\pm$ 0.12\\ 
& F763M&&&& 0.67 $\pm$ 0.10&\\ 
180916& F110W& 7.760 $\pm$ 0.023& 5.386$ \pm$ 0.016& 0.897 $ \pm$ 0.003& 0.32 $\pm$ 0.07&0.90 $\pm$ 0.09\\ 
& F673N&&&& 0.32 $\pm$ 0.25&\\ 
180924& F160W& 0.71 $\pm$ 0.12& 3.37$ \pm$ 0.56& 1.20 $ \pm$ 0.20& 0.24 $\pm$ 0.11&0.66 $\pm$ 0.07\\ 
& F300X&&&&&\\ 
190102& F160W& 0.80 $\pm$ 0.39& 2.26$ \pm$ 2.22& 0.45 $ \pm$ 0.44& 0.39 $\pm$ 0.25&0.25 $\pm$ 0.16\\ 
& F300X&&&& 0.36 $\pm$ 0.29&\\ 
190608& F160W& 2.98 $\pm$ 0.27& 6.52$ \pm$ 0.60& 0.88 $ \pm$ 0.08& 0.19 $\pm$ 0.06&0.82 $\pm$ 0.08\\ 
& F300X&&&& 0.39 $\pm$ 0.28&\\ 
190611& GMOS-S$_r$& 2.24 $\pm$ 0.66& 11.36$ \pm$ 3.59& 5.29 $ \pm$ 1.67&&\\ 
&&&&&&\\ 
190711& F160W& 0.53 $\pm$ 0.27& 1.94$ \pm$ 2.30& 0.78 $ \pm$ 0.93& 0.55 $\pm$ 0.27&0.61 $\pm$ 0.22\\ 
& F300X&&&&&\\ 
190714& F160W& 0.61 $\pm$ 0.29& 1.97$ \pm$ 1.18& 0.51 $ \pm$ 0.31& 0.34 $\pm$ 0.23&0.23 $\pm$ 0.10\\ 
& F300X&&&& 0.38 $\pm$ 0.31&\\ 
191001& F160W& 2.74 $\pm$ 0.15& 10.49$ \pm$ 0.59& 2.87 $ \pm$ 0.16& 0.09 $\pm$ 0.03&0.91 $\pm$ 0.09\\ 
& F300X&&&& 0.29 $\pm$ 0.25&\\ 
200430& Pan-STARRS$_r$& 1.30 $\pm$ 0.79& 2.97$ \pm$ 2.36& 1.81 $ \pm$ 1.44&&\\ 
&&&&&&\\ 
\hline 
Median (IR) & & 1.1 & 3.2 & 0.9 & 0.33 & 0.6 
\\ 
16,84\% Interval & & [0.6,2.9] & [2.0,8.7] & [0.5,2.4] & [0.20,0.53] & [0.2,0.9]  
\\ 
Median (UV) & &  &  & & 0.37  
\\ 
16,84\% Interval & &  &  &  & [0.32,0.45]  
\\ 
\hline 
\enddata 
\tablecomments{FRBs\,190611 and 200430 are derived from ground-based imaging as reported in \citet{Heintz20}} 
\end{deluxetable*} 

